iServe: An Intent-based Serving System for LLMs

Large Language Models (LLMs) are becoming ubiquitous across industries, where applications demand they fulfill diverse user intents. However, developers currently face the challenge of manually exploring numerous deployment configurations - combinations of parallelism and compression techniques that impact resource usage, latency, cost, and accuracy - to meet these intents. Assessing the impact of these configurations on user metrics requires extensive, costly profiling for each model. Existing approaches avoid this expense by using fixed, static configurations, but this often leads to sub-optimal performance and higher costs. Moreover, none of these solutions dynamically adapt to changing user intents to balance latency and cost, effectively. We present iServe, an automated, intent-based system for distributed LLM inference. Instead of manually selecting deployment configurations, developers simply specify their intent - such as minimizing latency, reducing cost, or meeting specific targets for either. iServe introduces fingerprints, lightweight representations of LLMs, to efficiently estimate how different configurations impact latency and memory usage. Based on these insights and GPU availability, iServe dynamically selects the optimal configuration to align with the user's intent. For various LLMs and query arrival rates, iServe best meets user intents compared to state-of-the-art systems by reducing latency by 77.62% and SLO violations by 7.09x while improving GPU throughput by 4.72x. Moreover, iServe's fingerprint-based profiling reduces profiling cost by 6.05x (GPU-hours) compared to baselines.

==> 1_OLD_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\noindent\textbf{Motivation.} 
%Inference from Large Language Models (LLMs) is significantly impacting several domains, including healthcare~\cite{peng2023study}, education~\cite{su151612451}, and finance~\cite{math10132156, li2023large}. %, ~\cite{li2023large}. 
%In addition to the rapidly increasing capabilities of LLMs, ease of use offered by platforms like HuggingFace~\cite{huggingface}, PyTorch Hub~\cite{pytorch-hub}, and compute capabilities offered by GPU cloud instances~\cite{lambdalabs} are key enablers of wide adoption of LLMs.
%However, such 
Rapidly growing reliance on inference from Large Language Models (LLMs) across various domains, including healthcare~\cite{peng2023study}, education~\cite{su151612451}, and finance~\cite{math10132156, li2023large}, demands capabilities that far exceed that of modern accelerators.
For example, between 2018 and 2022, the size of LLMs grew by $1600\times$ (BERT-large~\cite{devlin2019bert} vs. PaLM~\cite{chowdhery2022palm}), whereas GPU memory only grew by $5\times$ (V100~\cite{nvidia_2018} vs. H100~\cite{nvidia_2022}). 
%To bridge this gap, a plethora of techniques, including model compression and parallelism, exist \neeraja{citations}. 
%Existing inference \neeraja{citations here} serving systems either statically fix the combination of these techniques or force users to choose the combination to meet application needs. Both result in suboptimal performance and cost for users.
%The advent of large language models (LLMs) has revolutionized AI, as LLMs offer unprecedented capabilities in understanding and generating text. Notably, LLMs have permeated several domains aside from machine learning (ML), including healthcare~\cite{peng2023study}, education~\cite{su151612451}, and finance~\cite{math10132156}, ~\cite{li2023large}. This is because \emph{non-expert} users can easily download and deploy LLMs within minutes using platforms like Hugging Face~\cite{huggingface}, PyTorch Hub~\cite{pytorch-hub}, and GPU cloud instances~\cite{lambdalabs}. However, a key deployment challenge users face is efficiently handling the growing sizes of LLMs; as LLMs continue to improve, their rate-of-growth far exceeds that of modern GPU memory. For example, between 2018 and 2022, the size of LLMs grew by $1600\times$ (BERT-large~\cite{devlin2019bert} vs. PaLM~\cite{chowdhery2022palm}), whereas GPU memory only grew by $5\times$ (V100~\cite{nvidia_2018} vs. H100~\cite{nvidia_2022}). % \prasoon{TODO: Tianrui and Dimitris, please fill out $x$ above and add citations.}\dimitrios{DONE}
%To handle the growing size of LLMs, \emph{expert} users (e.g., ML practitioners) employ a plethora of techniques introduced by the ML community when deploying LLMs.

To bridge the gap between the growing size of LLMs and accelerator capabilities, ML experts introduced a plethora of techniques to deploy LLMs.
Model parallelism techniques (e.g., data~\cite{shallue2019measuring}, pipeline~\cite{huang2019gpipe}, and tensor parallelism~\cite{Wang_2022}) %enable users to 
distribute these large models across multiple GPUs.
Model compression techniques (e.g., quantization, pruning) reduce the size of large models.
% \prasoon{TODO: Tianrui and Dimtris, please fill out the technique names for quantization and pruning, and include the citations to each below.} \tianrui{Done}
Quantization techniques~\cite{dettmers2022llmint8, frantar2023gptq, xiao2023smoothquant, dettmers2023qlora, Yu20248bit, lin2023awq} lower the bit-width (e.g., 16-bit to 8-bit, 16-bit to 4-bit) of LLM weights and activations thereby reducing memory needed~\cite{wang2024decodingtrust}.
%Quantization techniques, including LLM.int8()~\cite{dettmers2022llmint8}, GPTQ~\cite{frantar2023gptq}, SmoothQuant~\cite{xiao2023smoothquant}, QLoRa~\cite{dettmers2023qlora}, Posit8~\cite{Yu20248bit} and AWQ~\cite{lin2023awq}, lower the bit-width (e.g., 16-bit to 8-bit, 16-bit to 4-bit) of LLM weights and activations thereby reducing memory needed~\cite{wang2024decodingtrust}. %without significant impact on output quality~\cite{wang2024decodingtrust}.
These techniques have also been applied to reduce the size of the large KV-cache of LLMs~\cite{int8kvcache, dong2024qaq}.
% Quantization techniques, including x[], y[], and z[], intelligently lower the bit-width (e.g., 16-bit to 8-bit) of LLM weights by blah \prasoon{Tianrui and Dimitris, please explain succintly how these techniques intelligently reduce bit-width.}.
Pruning techniques~\cite{frantar2023sparsegpt, sun2023wanda, ma2023llmpruner} use various algorithms to identify and remove insignificant weights and layers in LLMs. % , remove them in a given proportion. %, and then restore the model's performance with a small dataset. 
\begin{figure}[t]
     \centering
     \includegraphics[width=\linewidth]{Figures/1.Introduction/Figure1.pdf}
     \vspace{-5mm}
     \caption{%\neeraja{D\&T: Get rid of the "Minimization goal" from the figure.} \tianrui{Done} \neeraja{P, explain what PP, TP, OOM etc., is in the caption.} \prasoon{Done}
     Normalized inference latency and cost for Falcon-40B and GPT-J-6B under different tensor parallelism (TP) and pipeline parallelism (PP) degrees. The optimal parallelism configuration is specific to the model and end goal.    
     % Normalized latency and costs for serving 50-token outputs using the Falcon-40B model with Float16 weights and the GPT J-6B model with INT4 weights on an RTX A6000 across various parallelism configurations. The optimal configuration for minimizing costs with the GPT J-6B cannot be applied to the Falcon-40B. Similarly, the best configuration for minimizing latency with the Falcon-40B increases both latency and cost for the GPT J-6B.
     }
     \label{fig:introduction}
 \end{figure}

% These model parallelism and compression techniques can
% be used in combination with each other; a single LLM can
% be quantized and have a mix of pipeline and tensor paral-
% lelism, for example. Such combinations of these techniques
% result in a large number of ways an LLM can be deployed;
% we refer to such combinations as deployment configurations.
% For example, Llama2-70B can be deployed with tensor paral-
% lelism degree of 4, pipeline parallelism degree of 2, activation
% weights quantization of int4, and KV-cache quantizaiton of
% int8.

Model parallelism and compression techniques can be leveraged together. 
For example, Llama2-70B can be deployed with tensor parallelism degree of 4, pipeline parallelism degree of 2, activation weights quantization of int4, and KV-cache quantization of int8.
We refer to such a combination as an LLM's \emph{deployment configuration}.
With multiple options per configuration parameter, the combination of deployment techniques creates a vast number of LLM deployment options.
%\neeraja{Give an example of a configuration here to make sure a reader understands what we mean by a deployment configuration} 
%\prasoon{Done}
% \prasoon{Neeraja, there is more to a deployment configuration than just the parallelism degrees. Also the type of quantization of the weights and the quantization of KV cache. Hence, not sure if it makes sense to give the example here.} 
%\tianrui{Here, the pipeline parallelism can assign a different number of layers to each device, which means it is more complex than simply saying pp = x}
%For example, a configuration can be ${pipeline parallelism level = 2, tensor parallelism level = 4, weight quantization = INT4, KV cache quantization = INT8}$, which means deploying the LLM using pipeline parallelism to assign layers of the LLM to two sets of devices, and then splits the matrices of the LLM in each set into four devices. All the weights 
Moreover, the choice of hardware resources (e.g., different types of GPUs) and differences across model architectures increase this space of configurations.
For example, Llama2-70B\footnote{Llama2-70B has 15 model parallelization choices (4 degrees of tensor and 8 degrees of pipeline parallelism), 4 quantization choices for activation weights (assuming the use of well-tested, stable quantization techniques), 2 quantization choices for the KV-cache, and 4 pruning choices.} in an 8-GPU cluster results in up to 480 deployment configurations that impact various metrics in a significant way.
For instance, to generate 100 tokens using these configurations of Llama2-70B, inference latency ranges from $2.58$ to $22.02$ seconds ($8.54\times$), total memory consumption ranges from $32.12$ to $141.23$ GB ($4.40\times$), user cost ranges from $\$0.00038$ to $\$0.0115$ ($30.04\times$)~\cite{runpod}, and GPU time consumed ranges from $7.33$ to $174.37$ seconds ($23.78\times$).
Thus, \emph{the choice of a deployment configuration for an LLM is key in achieving the desired latency and cost for users.} % remains a key problem.
%Existing inference \neeraja{citations here} \tianrui{DONE}~\cite{aminabadi2022deepspeed},~\cite{tensorrt-llm},~\cite{lin2023superscaler},~\cite{oh2024exegpt} serving systems either statically fix the combination of these techniques or force users to choose the combination to meet application needs. 

\noindent\textbf{Challenges.}
Given the large configuration space, the key challenge in selecting a deployment configuration for an LLM is determining the impact of each deployment configuration on user metrics (e.g., the expected latency for a given configuration). 
%The key challenge in leveraging various parallelism and compression techniques for LLM deployment is determining the impact of each deployment configuration on user metrics (e.g., the expected latency for a given configuration). 
As Figure~\ref{fig:introduction} shows, there is no single deployment configuration that is consistently best across LLMs and/or across user metrics (e.g., latency. cost).
Hence, extensive and expensive profiling of each LLM is required to learn this relationship.
For example, it took 5.46 hours, 8 GPUs, 5.68 TB of GPU memory, and 32.02 GPU-hours to profile 80 of the 120 Llama2-70B deployment configurations.
%\neeraja{Prasoon, bring out the key challenges of profiling here. We just established so far that there are too many configurations and that they have significant impact on user metrics. Now, talk about the challenge of figuring out the relationship between a deployment configuration and the impact on these metrics (meaning what latency to expect from a given configuration, etc. This leads to extensive and expensive profiling of each LLM for every possible configuration -- give example here as to how much memory, time, and gpu-hours this would mean for an example model, might be better to continue with the running example of llama-70B. This should then connect to the following para about existing work that simply fixes configurations across models or leaves it to users to specify the configurations for each model.}
%\prasoon{Done}
%\dimitrios{Experiment Setup: 8 x A6000, Configurations: MODEL: llama-2-70b, DTYPE: ['float16' 'int4' 'int4\_gptq' 'int8'], KV-CACHE-INT8: [False  True], TP-SIZE: [1 2 4 8], PP-SIZE: [1 2 3 4 5 6 7 8]. 
%Model: llama-2-70b --> Num of configs: 80, Sum Naive Time: 5.46 hours, Sum Naive Memory: 5.68 TB, Sum Naive GPU Time: 32.02 hours. The number of possible configurations here is 80 because tp-deg x pp-deg must be at most 8, and the model has to be able to fit in the selected gpus (eg. tp=1, pp=1, dtype=float16 cannot be used), those are the only constrains.}

\noindent\textbf{Prior work.} Given this severe overhead involved in profiling, existing inference serving systems, including those introduced by academia (SpotServe~\cite{miao2023spotserve}, DeepSpeed~\cite{aminabadi2022deepspeed}, Tensorrt-LLM~\cite{tensorrt-llm}) and industry (Accelerate~\cite{huggingface}, PyTorch~\cite{pytorch-hub}, and JAX~\cite{jax}), 
either fix the model parallelization technique across different models~\cite{oh2024exegpt} or leave it to users to specify the deployment configuration~\cite{aminabadi2022deepspeed, tensorrt-llm, lin2023superscaler}. 
Both result in suboptimal performance and cost for users, as (1) different LLMs require different deployment configurations depending on the user goal (Figure~\ref{fig:introduction}) and status of available resources in GPU clusters, and (2) making a choice of configuration requires understanding of the internals of the model and hardware accelerators that non-expert users may not have. 

%While effective in efficiently deploying LLMs, it is challenging for \emph{non-expert} users to choose the combination of model parallelism and compression techniques to meet their requirements.
%For example, Llama2-70B\footnote{Llama2-70B has 32 model parallelization choices, 4 quantization choices for activation weights (assuming the use of well-tested, stable quantization techniques), 2 quantization choices for the KV-cache, and 4 pruning choices.} deployed on an 8-GPU cluster has up to 1024 deployment configurations alone.
%To generate 100 tokens, These variants vary across many dimensions: inference latency ranges from $2.58$ to $22.02$ ($8.54\times$), total memory consumption ranges from $32.12$ to $141.23$ ($4.40\times$), user cost ranges from $95.99$ to $2883.69$ ($30.04\times$), and GPU hours consumed ranges from $7.33$ to $174.37$ ($23.78\times$).
%Hence, LLM users have to navigate a large search-space to efficiently deploy LLMs that meet their user objective (e.g., latency, cost). 

%In the last few years, several LLM-based inference serving systems have been proposed to aid users in efficient LLM deployment. 
%Existing inference serving systems either fix the model parallelization technique~\cite{oh2024exegpt} or require users to specify the technique~\cite{aminabadi2022deepspeed},~\cite{tensorrt-llm},~\cite{lin2023superscaler}. 
%These systems include those proposed by both researchers (e.g., SpotServe~\cite{miao2023spotserve}, DeepSpeed~\cite{aminabadi2022deepspeed}, Tensorrt-LLM~\cite{tensorrt-llm}) and industry (e.g., Accelerate~\cite{huggingface}, PyTorch~\cite{pytorch-hub}, and JAX~\cite{jax}).
%\prasoon{TODO: Tianrui and Dimtris, please provide two plots, side by side. Left plot shows latency on y-axis, two LLMs on x-axis, three bars per LLM (one per deployment configuration of TP/PP level). Right plot shows cost on y-axis, two LLMs on x-axis, three bars per LLM (one per deployment configuration of TP/PP level). Choose two LLMs that have different deployment configurations that minimize latency and cost. I would suggest Llama2-13B and Falcon-7B.}
%However, static parallelization decisions are suboptimal, as (1) different LLMs require different deployment configurations depending on the user goal (Figure~\ref{fig:introduction}), and (2) the optimal deployment configuration may not be feasible (i.e., not enough GPUs) in a realistic GPU clusters where LLMs enter and leave dynamically.Moreover, systems requiring the specification of parallelization techniques are challenging for \emph{non-expert} users to leverage, as the search space is large and nontrivial to navigate.
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/1.Introduction/introduction_search_space.png}
%     \caption{Breakdown of possible configurations for a given LLM; different colors indicate different selected compression techniques (Comp-i), while PP-j and TP-k correspond to the pipeline and tensor parallelism degree. Each colored block in the last column is a part of the original model that has to loaded on a separate GPU.}
%     \label{fig:introduction_search_space}
% \end{figure}

A few recent systems automatically choose the optimal parallelization technique per LLM (e.g., AlpaServe~\cite{li2023alpaserve}, Galvatron~\cite{Galvatron2022}, Vidur~\cite{Agrawal2024}).
% \dimitrios{Vidur is a ML-for-SYS used to make prediction, can we put it here or it needs a separate category?} \tianrui{no, I believe the whole story is still the Sys for LLM.}
% \prasoon{Tianrui and Dimitris, please say a one sentence more insightful description of what theses systems do to make automatic parallelization decisions}. 
However, most of these systems (a) require knowledge of the future inference request arrivals~\cite{li2023alpaserve, Agrawal2024} that is not available in real-world settings,
%and operate on fixed workloads; i.e., they cannot handle the dynamic entering and leaving of LLMs in a GPU cluster.
(b) rely on heavy offline profiling that requires dedicated GPU resources, long-running simulations, or code changes~\cite{Agrawal2024} with the use of GPU toolchains, which may not be easy for general-purpose systems serving the LLMs for \emph{non-expert} users, 
%, where (1) they require a small dedicated cluster of GPUs for offline profiling, and (2) use either simulators that take tens of minutes to execute per LLM~\cite{li2023alpaserve} or require source code changes~\cite{Agrawal2024} with the use of GPU toolchains, which may not be easy for general-purpose systems serving the LLMs of \emph{non-expert} users.
(c) focus only on a subset of the deployment configuration search space (ignoring compression techniques)%; we find that the compression technique %and the number of GPUs 
%(\S~\ref{sec:background}) can significantly affect LLM performance.
and finally, (d) have a singular focus: AlpaServe~\cite{li2023alpaserve} maximizes SLO-attainment while Vidur minimizes cost~\cite{Agrawal2024}.
These systems do not dynamically adjust to different user requirements.

%\begin{comment}

%\neeraja{Commenting the following para from the intro. It is getting too late to talk about our work, so bringing that in here. Find a different place in later sections for the following para.}
\noindent\textbf{Our Work.} 
We build {\system}, a distributed inference serving system for LLMs that selects the optimal deployment configuration indicating parallelization techniques(s), compression technique(s), and number of GPUs to be used
given the dynamic state of the available GPUs to meet the user's goal (e.g., minimize latency, cost, memory, or GPU-hours).
To tackle the challenge of severe profiling costs mentioned earlier, {\system} leverages a key observation: commonly used LLMs -- the decoder-based LLMs including GPT-J~\cite{gptj}, Llama-2~\cite{touvron2023llama}, Falcon~\cite{almazrouei2023falcon}, Mixtral MoE~\cite{jiang2024mixtral} %\neeraja{add citations for each of these} \dimitrios{Done} 
-- consist of multiple hidden layers with the \emph{same structural components}. 
We introduce \emph{{\submodel}}, a reconstructed model that consists of the same building components (embedding layers, hidden blocks, linear layer and softmax activations) as the original model, but has only one or two hidden blocks. 
Thus, a {\submodel} captures the essence of the entire model but is significantly lightweight. 
For instance, the memory footprint of Llama-2-70B's fingerprint is only 3.28\% %\dimitrios{This is the 2-layer {\submodel}, should we specify it?} 
of the entire LLM's.
%\neeraja{Prasoon: Give the Llama-70B example here.}
%\prasoon{Done.}
Instead of profiling the entire model, we profile its {\submodel} on a small set of configurations and use the observed latency and memory to estimate the latency and memory required for the entire model for a given deployment configuration.
%\neeraja{Need a sentence or two here about how we really go from the measurements for the {\submodel} to the memory and latency estimates for the entire model given any deployment configuration. Prasoon, there is a long thread where Dimitris explined this but I am right now running out of time. Can you take a stab at tersely describing this? Don't need all the details, but rather intuitive explanation of the technical detail here. Section 5 needs to get all the details out, still in a readable way.}
Finally, unlike previous systems that require dedicated offline GPUs for profiling, {\system} utilizes a fraction of the free GPUs in its inference serving cluster to profile each user's LLM \emph{within minutes} without any code changes.



%We argue for a \emph{user-friendly} inference serving system that accounts for GPU cluster state (e.g., how many GPUs are free, how many models are loaded), \emph{automatically} determines the optimal deployment configuration (parallelization techniques(s), compression technique(s), and number of GPUs), and \emph{adjusts} to different user requirements (e.g., cost, latency) per LLM.
%The key challenge in building such a system is \emph{efficiently} navigating the large search space of deployment configurations.
%\neeraja{here, introduce the concept of fingerprints and how we use them to drastically bring the profiling overheads down while being accurate.}
%\prasoon{We do that in two paragraphs, do we still want it here?}
% For example, Llama2-70B deployed on an 8-GPU cluster has 1024 \dimitrios{If we take into account the PP distribution of layers across all pipelines, this number becomes even larger} deployment configurations alone\footnote{Llama2-70B has 32 model parallelization choices, 4 quantization choices for activation weights (assuming the use of well-tested, stable quantization techniques), 2 quantization choices for the KV-cache, and 4 pruning choices.}. 

%\end{comment}


%To that end, 
%We introduce {\system}, a distributed inference serving system for LLMs where: %user-friendly inference serving system for LLMs.
%(a) Users provide {\system} their LLMs along with an optimization goal (e.g., minimize latency, cost, memory, or GPU hours).
%(b) {\system} then automatically chooses the best deployment configurations to meet the user's goal given the state of the GPU cluster (e.g., how many GPUs are free, how many models are loaded).
%To do so, {\system} \emph{efficiently} constructs a lookup table per LLM consisting of the latency and memory requirements for \emph{each deployment configuration} and chooses the best, feasible configuration given the available resources in the GPU cluster to meet the user goal.

%Unlike previous systems that require dedicated offline GPUs for profiling, {\system} utilizes a fraction of the free GPUs in its inference serving cluster to profile each user's LLM \emph{within minutes} without any code changes.
%The key challenge in building such a system is \emph{efficiently} navigating the large search space of deployment configurations.
%{\system} leverages our key insight: decoder-based LLMs consist of multiple hidden layers with the same structural components -- we call these the \emph{{\submodel}} of the LLM.
%Hence, {\system} simply constructs and profiles these lightweight {\submodel}s of each LLM consisting of only one or two replicas of its unique layers.
%It leverages the profiled latency and memory values along with novel, handcrafted algorithms to estimate the latency and memory requirements \emph{for every deployment configuration} per LLM.


% We leverage the characteristics of the LLM to create a lightweight variant of the original model that consists of the same building blocks but has only one or two hidden layers. We profile these variants and record their end-to-end latency and memory usage. Then, we use two different algorithms, one for latency (\S~\ref{sec:background}) and one for memory (\S~\ref{sec:background}), to estimate the latency and memory usage for the entire LLM. We create the profiling datasets based on these estimations, and we use them to determine the most optimal configuration for deployment.
% \prasoon{TODO: Tianrui and Dimitris, please provide a paragraph on how many GPUs you evaluate on, what type of GPUs, and your gains per optimization goal compared to state-of-the-art baselines. Look at AlpaServe's last paragraph in the introduction for inspiration.}

% \prasoon{For results, I would provide the following: (1) }
%We build {\system} on top of NVIDIA TensorRT-LLM. We evaluate {\system} using both real and synthetic LLM traces on an 8-GPU cluster with pairwise NVLink-connected RTX A6000s. 

\noindent\textbf{Contributions.}
Our key contributions include:
\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item We present a detailed analysis of the trade-off space between latency and memory of different deployment configurations for LLMs.
\item We introduce LLM \emph{{\submodel}s}, unique layers that form the structural components that repeat themselves, and develop a novel profiling algorithm using these LLM {\submodel}s that accurately estimates latency and memory usage for LLM inference serving with minimal cost. % and corresponding on-fleet profiler.
\item We build \system, an LLM serving system that selects best configurations based on various user-defined policies in a dynamic GPU environment. 
%A comprehensive evaluation of {\system} with both synthetic and production traces. 
Our evaluation, using synthetic and production traces, shows that {\system} can achieve $3.50\times$ less memory use and $2.28\times$ less GPU usage per model while serving request rates $2.4\times$ higher compared to current serving systems.
\end{itemize}






















==> 1_new-intro-copy.tex <==
\section{Introduction}
\label{sec:introduction}

\begin{comment}
* LLMs everywhere, but the applications demand LLMs to meet varied user intents, give examples.
    * to satisfy these intents: parallelism, compression, etc.
    * these create a large search space, hard to navigate, requires expertise
* existing LLM inference serving systems fall short
* our work
\end{comment}

Large Language Models (LLMs) are ubiquitous across industries today where applications demand that they meet varied user intents. 
For instance, real-time chatbots and voice assistants prioritize low latency to deliver instant responses while education platforms and automated FAQs focus on cost-efficiency.
Meanwhile, mobile apps and IoT devices require minimal GPU usage.
To satisfy these diverse intents, experts introduced various (a) compression techniques that reduce the size of the models (e.g., quantization~\cite{} \neeraja{cite}, pruning~\cite{} \neeraja{cite}) and (b) parallelism techniques that distribute the models across multiple GPUs (e.g.,  data~\cite{shallue2019measuring}, pipeline~\cite{huang2019gpipe}, and tensor parallelism~\cite{Wang_2022}).
However, despite existing work in LLM inference serving, developers must manually search through hundreds of deployment configurations --- combinations of these techniques that differ in hardware, resource footprints, latencies, costs, and accuracies --- to satisfy the user intents.

%The combination of these techniques, along with the choice of hardware resources, results in many ways an LLM can be deployed. These deployment configurations vary across user metrics such as latency and cost, creating a large search space that requires expertise to navigate. 

%If we want to enable 
%Unfortunately, none of the existing LLM serving systems can automatically select a deployment configuration that aligns with specific user intents, making manual optimization essential.

\begin{comment}
%\noindent\textbf{Motivation.} 
%Inference from Large Language Models (LLMs) is significantly impacting several domains, including healthcare~\cite{peng2023study}, education~\cite{su151612451}, and finance~\cite{math10132156, li2023large}. %, ~\cite{li2023large}. 
%In addition to the rapidly increasing capabilities of LLMs, ease of use offered by platforms like HuggingFace~\cite{huggingface}, PyTorch Hub~\cite{pytorch-hub}, and compute capabilities offered by GPU cloud instances~\cite{lambdalabs} are key enablers of wide adoption of LLMs.
%However, such 
Rapidly growing reliance on inference from Large Language Models (LLMs) across various domains %, including healthcare~\cite{peng2023study}, education~\cite{su151612451}, and finance~\cite{math10132156, li2023large}, 
demands capabilities that far exceed that of modern accelerators.
For example, between 2018 and 2022, the size of LLMs grew by $1600\times$ (BERT-large~\cite{devlin2019bert} vs. PaLM~\cite{chowdhery2022palm}), whereas GPU memory only grew by $5\times$ (V100~\cite{nvidia_2018} vs. H100~\cite{nvidia_2022}). 
%To bridge this gap, a plethora of techniques, including model compression and parallelism, exist \neeraja{citations}. 
%Existing inference \neeraja{citations here} serving systems either statically fix the combination of these techniques or force users to choose the combination to meet application needs. Both result in suboptimal performance and cost for users.
%The advent of large language models (LLMs) has revolutionized AI, as LLMs offer unprecedented capabilities in understanding and generating text. Notably, LLMs have permeated several domains aside from machine learning (ML), including healthcare~\cite{peng2023study}, education~\cite{su151612451}, and finance~\cite{math10132156}, ~\cite{li2023large}. This is because \emph{non-expert} users can easily download and deploy LLMs within minutes using platforms like Hugging Face~\cite{huggingface}, PyTorch Hub~\cite{pytorch-hub}, and GPU cloud instances~\cite{lambdalabs}. However, a key deployment challenge users face is efficiently handling the growing sizes of LLMs; as LLMs continue to improve, their rate-of-growth far exceeds that of modern GPU memory. For example, between 2018 and 2022, the size of LLMs grew by $1600\times$ (BERT-large~\cite{devlin2019bert} vs. PaLM~\cite{chowdhery2022palm}), whereas GPU memory only grew by $5\times$ (V100~\cite{nvidia_2018} vs. H100~\cite{nvidia_2022}). % \prasoon{TODO: Tianrui and Dimitris, please fill out $x$ above and add citations.}\dimitrios{DONE}
%To handle the growing size of LLMs, \emph{expert} users (e.g., ML practitioners) employ a plethora of techniques introduced by the ML community when deploying LLMs.
To bridge this gap, experts introduced (a) compression techniques to reduce the size of the models (e.g., quantization, pruning) and (b) parallelism techniques to distribute the models across multiple GPUs (e.g.,  data parallelism~\cite{shallue2019measuring}, pipeline parallelism~\cite{huang2019gpipe}, and tensor parallelism~\cite{Wang_2022}).
\end{comment}

%However, a combination of these techniques along with the choice of hardware resources, called an LLM deployment configuration, is often required to meet the user intent.



The combination of these techniques, along with the choice of hardware resources, results in many ways in which an LLM can be deployed. 
%For example, Llama2-70B can be deployed with tensor parallelism degree of 4, pipeline parallelism degree of 2, activation weights quantization of int4, and KV-cache quantization of int8.
%We refer to such a combination as an LLM's \emph{deployment configuration}.
%Moreover, the choice of hardware resources %(e.g., different types of GPUs) 
%and differences across model architectures increase this space of configurations.
For example, Llama2-70B can be deployed in 480 different ways on an 8-GPU cluster (Figure~\ref{fig:llama-70b-search-space}): 15 ways to parallelize (4 degrees of tensor and 8 of pipeline parallelism), 4 ways to quantize the weights, 2 ways to quantize the KV-cache, and 4 ways to prune. 
%These deployment configurations vary across many dimensions: to generate 100-token outputs, inference latency ranges from $2.58$ to $22.02$ seconds ($8.54\times$), total memory consumption ranges from $32.12$ to $141.23$ GB ($4.40\times$), user cost ranges from $\$0.00038$ to $\$0.0115$ ($30.04\times$), and GPU time consumed ranges from $7.33$ to $174.37$ GPU-seconds ($23.78\times$).
These deployment configurations vary across many dimensions: inference latency ranges from $2.58$ to $22.02$ seconds ($8.54\times$), total memory consumption ranges from $32.12$ to $141.23$ GB ($4.40\times$), GPU time consumed ranges from $7.33$ to $174.37$ GPU-seconds ($23.78\times$), and based on the Azure LLM serving trace~\cite{patel2024splitwise}, during one hour of handling requests with 100-token outputs, user cost ranges from $\$7.36$ to $\$222.07$ ($30.04\times$).
%\tianrui{Here is the data from Azure: These deployment configurations vary across many dimensions: inference latency ranges from $2.58$ to $22.02$ seconds ($8.54\times$), total memory consumption ranges from $32.12$ to $141.23$ GB ($4.40\times$), GPU time consumed ranges from $7.33$ to $174.37$ GPU-seconds ($23.78\times$), and based on the Azure LLM serving trace~\cite{patel2024splitwise}, during a one-hour period of handling requests with 100-token outputs, user cost ranges from $\$7.36$ to $\$222.07$ ($30.04\times$).}
%For instance, to generate 100 tokens using these configurations of Llama2-70B, inference latency ranges from $2.58$ to $22.02$ seconds ($8.54\times$), total memory consumption ranges from $32.12$ to $141.23$ GB ($4.40\times$), user cost ranges from $\$0.00038$ to $\$0.0115$ ($30.04\times$)~\cite{runpod}, and GPU time consumed ranges from $7.33$ to $174.37$ seconds ($23.78\times$).
Thus, \emph{the choice of a deployment configuration for an LLM is key in meeting varied user intents .} %achieving the desired latency and cost for users.}

% \begin{figure}[t]
%      \centering
%      \includegraphics[width=1.05\linewidth]{Figures/1.Introduction/Figure1.pdf}
%      \vspace{-5mm}
%      \caption{%\neeraja{D\&T: Get rid of the "Minimization goal" from the figure.} \tianrui{Done} \neeraja{P, explain what PP, TP, OOM etc., is in the caption.} \prasoon{Done}
%      Normalized inference latency and cost for Falcon-40B and GPT-J-6B under different tensor parallelism (TP) and pipeline parallelism (PP) degrees. The optimal parallelism configuration is specific to the model and end goal.    
%      % Normalized latency and costs for serving 50-token outputs using the Falcon-40B model with Float16 weights and the GPT J-6B model with INT4 weights on an RTX A6000 across various parallelism configurations. The optimal configuration for minimizing costs with the GPT J-6B cannot be applied to the Falcon-40B. Similarly, the best configuration for minimizing latency with the Falcon-40B increases both latency and cost for the GPT J-6B.
%      }
%      \label{fig:introduction}
%  \end{figure}

\begin{figure}[t]
     \centering
     \includegraphics[width=\linewidth]{Figures/1.Introduction/Search_space_llama70b.pdf}
     \vspace{-9mm}
     \caption{There are hundreds of deployment configurations per LLM with latency and memory consumption trade-offs. The optimal configuration is specific to the user intent.
     % Effect on memory footprint and serving latency of LLAMA-2-70B under different configurations. The optimal parallelism configuration is specific to the end goal.
     %\dimitrios{I prefer the 2-stage figure, but if you think that this is easier to show our point and is better to understand we can keep this}
     }
     \vspace{-10mm}
     \label{fig:llama-70b-search-space}
 \end{figure}

However, understanding the impact of deployment configurations on user metrics requires extensive and expensive profiling of each LLM. 
For example, it took 5.46 hours and 8 GPUs %, 5.68 TB of GPU memory, and 32.02 GPU-hours 
to profile 80 of the 145 Llama2-70B deployment configurations.
Prior work circumvents this cost either by fixing the model parallelism techniques across different models~\cite{oh2024exegpt, zheng2022alpa, duan2024mopar} or leaving it to users to specify the deployment configuration~\cite{aminabadi2022deepspeed, tensorrt-llm, lin2023superscaler, kwon2023vllm, Athlur2022Varuna, CTranslate2}.
Both result in sub-optimal performance and cost for users, as (1) the best deployment configuration is LLM-specific, intent-specific, and depends on the availability of resources in the GPU cluster (\S~\ref{sec:characterization}), and (2) understanding the implications of different combinations of configuration parameters (e.g., parallelism, quantization, pruning) requires expert-level understanding of LLM architectures and hardware accelerators, which many LLM users do not have.
% different LLMs require different deployment configurations depending on the user goal (Figure~\ref{fig:introduction}) and status of available resources in GPU clusters, and (2) making a choice of configuration requires understanding of the internals of the model and hardware accelerators that non-expert users may not have. 
A few recent systems attempt to automatically navigate the deployment configuration search space by narrowing it to only parallelism techniques~\cite{li2023alpaserve, Galvatron2022, Agrawal2024, miao2023spotserve, Lin2024QUART, oh2024exegpt}.
However, they (1) assume knowledge of future query arrival patterns~\cite{li2023alpaserve, Agrawal2024}, (2) require code changes to the LLM~\cite{Agrawal2024}, and/or (3) rely on expensive profiling~\cite{li2023alpaserve}.
Lastly, \emph{none adapt to varying user intents to trade off latency vs cost.}
% While a few recent systems automatically choose parallelism technique for an LLM~\cite{li2023alpaserve, Galvatron2022, Agrawal2024}, they either assume knowledge of the future inference request arrivals or require code changes. %~\cite{Agrawal2024}.
% Lastly, \emph{none adapt to varying user requirements to trade off latency vs cost.}

\noindent\textbf{Our Work.} 
We build {\system}, a distributed LLM inference serving system that automatically deploys an LLM with the configuration---parallelism and compression technique(s)---that best meets the user intent.
{\system} exposes a rich interface to allow users to communicate their latency-cost trade-offs.

\neeraja{needs work.}
To efficiently navigate the large deployment configuration search space, we leverage our key observation: commonly used LLMs---decoder-based LLMs including GPT-J~\cite{gptj}, Llama-2~\cite{touvron2023llama}, Falcon~\cite{almazrouei2023falcon}, Mixtral MoE~\cite{jiang2024mixtral}---consist of multiple hidden layers with the \emph{same structural components}.
Using this insight, we introduce LLM \emph{fingerprints}, a reconstructed model that encompasses the same unique components (embedding layers, hidden layers, linear layers, softmax activations) as its LLM counterpart, but with at most two hidden layers (Figure~\ref{fig:fingerprint}).
Fingerprints capture the essence of the full LLM while being extremely lightweight: the memory footprint of Llama-2-70B's fingerprint is only 3.28\% of the entire LLM's.
Hence, instead of profiling the LLM, {\system} profiles its fingerprint on a small set of configurations and uses the profiled data to estimate the latency and memory requirements for every deployment configuration of an LLM.
Observing the fingerprint significantly reduces profiling cost (time and resources), enabling {\system} to harvest spare resources in the GPU cluster for profiling rather than requiring dedicated offline GPUs.

During deployment time, {\system} uses the LLM's estimated data to choose the configuration for an LLM that (a) is feasible to deploy given the availability of GPU memory in the cluster, and (b) best meets the user intent.
After, {\system} uses a load-aware LLM-to-GPU placement algorithm to map which GPUs to deploy the LLM onto; this algorithm balances packing LLMs onto fewer GPUs to improve utilization versus dispersing LLMs across GPUs to reduce contention.

We build {\system} on top of TensorRT-LLM, a popular LLM inference serving platform widely used in industry \cite{aws2024, alibaba2024, cerebrium2024, trtAmazon, trtAmex, trtZoox} and prior work \cite{li2023speedodysseydeployablequantization, li2022easyefficienttransformer, wu2024fastdistributedinferenceserving, kwon2023vllm, 280922}.
We evaluate {\system} against two static baselines and two state-of-the-art systems using two production-level LLM inference serving traces released by Azure \cite{patel2024splitwise}.
Across a range of LLMs and query arrival rates, {\system} best meets the user-intent: {\system} minimize latency by 31.86-99.90\%, cost by 67.06-99.79\%, and SLO violations by 3.03-7.09$\times$, all while increasing GPU throughput by 1.34-13.70$\times$ compared to the state-of-the-art systems, including 
AlpaServe~\cite{li2023alpaserve} and Accelerate~\cite{sylvain2022accelerate}. 

% We build {\system}, a distributed inference serving system for LLMs that selects a deployment configuration indicating parallelism techniques(s), compression technique(s), and number of GPUs to be used
% given the dynamic state of the available GPUs to meet the user's goal (e.g., minimize latency, cost, memory, or GPU-hours).

% To tackle the challenge of severe profiling costs mentioned earlier, {\system} leverages a key observation: commonly used LLMs -- the decoder-based LLMs including GPT-J~\cite{gptj}, Llama-2~\cite{touvron2023llama}, Falcon~\cite{almazrouei2023falcon}, Mixtral MoE~\cite{jiang2024mixtral} %\neeraja{add citations for each of these} \dimitrios{Done} 
% -- consist of multiple hidden layers with the \emph{same structural components}. 
% \prasoon{TOOD: add forward pointer to Figure 2 referring to fingerprint diagram.}
% We introduce \emph{{\submodel}}, a reconstructed model that consists of the same building components (embedding layers, hidden blocks, linear layer and softmax activations) as the original model, but has only one or two hidden blocks. 
% Thus, a {\submodel} captures the essence of the entire model but is significantly lightweight. 
% For instance, the memory footprint of Llama-2-70B's fingerprint is only 3.28\% %\dimitrios{This is the 2-layer {\submodel}, should we specify it?} 
% of the entire LLM's.
% %\neeraja{Prasoon: Give the Llama-70B example here.}
% %\prasoon{Done.}
% Instead of profiling the entire model, we profile its {\submodel} on a small set of configurations and use the observed latency and memory to estimate the latency and memory required for the entire model for a given deployment configuration.
% %\neeraja{Need a sentence or two here about how we really go from the measurements for the {\submodel} to the memory and latency estimates for the entire model given any deployment configuration. Prasoon, there is a long thread where Dimitris explined this but I am right now running out of time. Can you take a stab at tersely describing this? Don't need all the details, but rather intuitive explanation of the technical detail here. Section 5 needs to get all the details out, still in a readable way.}
% Finally, unlike previous systems that require dedicated offline GPUs for profiling, {\system} utilizes a fraction of the free GPUs in its inference serving cluster to profile each user's LLM \emph{within minutes} without any code changes.



%We argue for a \emph{user-friendly} inference serving system that accounts for GPU cluster state (e.g., how many GPUs are free, how many models are loaded), \emph{automatically} determines the optimal deployment configuration (parallelization techniques(s), compression technique(s), and number of GPUs), and \emph{adjusts} to different user requirements (e.g., cost, latency) per LLM.
%The key challenge in building such a system is \emph{efficiently} navigating the large search space of deployment configurations.
%\neeraja{here, introduce the concept of fingerprints and how we use them to drastically bring the profiling overheads down while being accurate.}
%\prasoon{We do that in two paragraphs, do we still want it here?}
% For example, Llama2-70B deployed on an 8-GPU cluster has 1024 \dimitrios{If we take into account the PP distribution of layers across all pipelines, this number becomes even larger} deployment configurations alone\footnote{Llama2-70B has 32 model parallelization choices, 4 quantization choices for activation weights (assuming the use of well-tested, stable quantization techniques), 2 quantization choices for the KV-cache, and 4 pruning choices.}. 

%\end{comment}


%To that end, 
%We introduce {\system}, a distributed inference serving system for LLMs where: %user-friendly inference serving system for LLMs.
%(a) Users provide {\system} their LLMs along with an optimization goal (e.g., minimize latency, cost, memory, or GPU hours).
%(b) {\system} then automatically chooses the best deployment configurations to meet the user's goal given the state of the GPU cluster (e.g., how many GPUs are free, how many models are loaded).
%To do so, {\system} \emph{efficiently} constructs a lookup table per LLM consisting of the latency and memory requirements for \emph{each deployment configuration} and chooses the best, feasible configuration given the available resources in the GPU cluster to meet the user goal.

%Unlike previous systems that require dedicated offline GPUs for profiling, {\system} utilizes a fraction of the free GPUs in its inference serving cluster to profile each user's LLM \emph{within minutes} without any code changes.
%The key challenge in building such a system is \emph{efficiently} navigating the large search space of deployment configurations.
%{\system} leverages our key insight: decoder-based LLMs consist of multiple hidden layers with the same structural components -- we call these the \emph{{\submodel}} of the LLM.
%Hence, {\system} simply constructs and profiles these lightweight {\submodel}s of each LLM consisting of only one or two replicas of its unique layers.
%It leverages the profiled latency and memory values along with novel, handcrafted algorithms to estimate the latency and memory requirements \emph{for every deployment configuration} per LLM.


% We leverage the characteristics of the LLM to create a lightweight variant of the original model that consists of the same building blocks but has only one or two hidden layers. We profile these variants and record their end-to-end latency and memory usage. Then, we use two different algorithms, one for latency (\S~\ref{sec:background}) and one for memory (\S~\ref{sec:background}), to estimate the latency and memory usage for the entire LLM. We create the profiling datasets based on these estimations, and we use them to determine the most optimal configuration for deployment.
% \prasoon{TODO: Tianrui and Dimitris, please provide a paragraph on how many GPUs you evaluate on, what type of GPUs, and your gains per optimization goal compared to state-of-the-art baselines. Look at AlpaServe's last paragraph in the introduction for inspiration.}

% \prasoon{For results, I would provide the following: (1) }
%We build {\system} on top of NVIDIA TensorRT-LLM. We evaluate {\system} using both real and synthetic LLM traces on an 8-GPU cluster with pairwise NVLink-connected RTX A6000s. 

% \noindent\textbf{Contributions.}
% We make the following contributions:
% % \vspace{-3mm}
% \begin{itemize}[leftmargin=*]%[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
% \item We present a detailed analysis of the trade-off space between latency and memory of different deployment configurations for LLMs.
% \item We introduce LLM \emph{{\submodel}s}, unique layers that form the structural components that repeat themselves, and develop a novel profiling algorithm using these LLM {\submodel}s that accurately estimates latency and memory usage for LLM inference serving with minimal cost. % and corresponding on-fleet profiler.
% \item We build \system, an LLM serving system that selects configurations to meet various user requirements. % in a dynamic GPU environment. 
% %A comprehensive evaluation of {\system} with both synthetic and production traces. 
% Our evaluation, using synthetic and production traces, shows that {\system} can achieve $3.50\times$ less memory use and $2.28\times$ less GPU usage per model while serving request rates $2.4\times$ higher compared to current serving systems including AlpaServe and Tensorrt-LLM \cite{huggingface, tensorrt-llm, li2023alpaserve}. \neeraja{name these systems here and add citations to them.} \tianrui{TODO: update this part with newest data from two different lists of models.}
% \end{itemize}







==> 3_design.tex <==
\section{{\system} Design}
\label{sec:design}
\tianrui{OLD version}
We leverage the takeaways from \S~\ref{sec:background} to design {\system}, a flexible LLM inference serving system that automatically selects the best LLM deployment configuration for a user's goal given the dynamic state of the GPU cluster.
In {\system}, a deployment configuration consists of a tensor parallelism (TP) degree, pipeline parallelism (PP) degree, technique used to quantize activation weights, and technique used to quantize the LLM's KV-cache.
{\system} supports four user objectives (minimize cost, latency, memory, or GPU-time) with its three main components:

\noindent\textbf{1. Fingerprint Generator.}
Leveraging the repetitive structure of LLM architectures (\S~\ref{sec:background}), %\neeraja{fix ref.} \dimitrios{Done}, 
the Fingerprint Generator creates a lightweight fingerprint of the LLM.
The fingerprint replicates the LLM's architecture, but removes most of the model's repeated hidden layers, making it significantly more lightweight.
We detail the FingerPrint Generator in \S~\ref{sec:generator_profiler}.

\noindent\textbf{2. Profiler.}
%The Profiler creates a small lookup table per LLM that stores the inference latency and memory requirements of each LLM deployment configuration. 
The Profiler collects key information (e.g., time-to-first-token (TTFT), TP memory overhead) for a given LLM using its fingerprint and maintains it in a lookup table for efficient access by the Model Deployer.
The Profiler uses spare memory available in the GPU cluster for profiling using the fingerprints.
%For a given LLM, the Profiler deploys the model's fingerprint on the spare memory available in the GPU cluster to profile key information (e.g., TTFT, TP memory overhead) and maintains this data in a small lookup table \emph{within minutes}.
We detail the Profiler in \S~\ref{sec:generator_profiler}.

\noindent\textbf{3. Model Deployer.}
The Model Deployer leverages the lookup table generated by the Profiler to choose the best deployment configuration to meet a user's goal. 
The Model Deployer accounts for the state of the GPU cluster (i.e., total available memory and available per-GPU memory) to ensure the configuration it picks is feasible to deploy.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/3.Design/design.pdf}
    \caption{Architecture of {\system}.}
    \label{fig:system_design}
\end{figure}

\pgfkeys{/csteps/inner color=white}
\pgfkeys{/csteps/fill color=black}

Figure~\ref{fig:system_design} describes {\system}'s workflow, split into two phases: the Model Registration and User Inference phase. 
Both phases leverage the same GPU cluster.
\Circled{1} A \emph{developer} provides their pre-trained LLM with model-specific information: model family (e.g., Llama2), model size (e.g., 70 billion parameters), and applicable quantization techniques (e.g., int8, GPTQ4).
\Circled{2} {\system}'s Fingerprint Generator creates a lightweight fingerprint of the LLM, which is used by \Circled{3} the Profiler to collect the inference latency and memory consumption of each LLM deployment configuration.
The Profiler deploys the fingerprint on the same cluster that serves user inferences.
We eliminate contention created from profiling by ensuring the profiling efforts are inexpensive in both latency and GPU memory consumption (\S~\ref{sec:eval_overhead}).
% and construct a lookup table with this information for each potential deployment configuration of the LLM.
% This completes the end of the Model Registration Phase.
\Circled{4} Once profiled, \emph{users} of {\system} can select registered models to deploy and specify their objective (e.g., minimize cost). 
\Circled{5} {\system}'s Model Deployer then uses an LLM's constructed lookup table to choose the configuration that meets the user's objective given the available GPU memory across the cluster.
\Circled{6} After deployment, users can submit inference queries, which a load balancer routes to the respective LLM.

\noindent\textbf{Inference Batch Sizes.}
Although batching inference requests can increase GPU utilization and total throughput, we target large models with small batches, which can fully utilize GPUs.
Small batches (batch size 1) mimic the behaviour of online LLM serving systems where queries are received and served in a sequential manner.
Hence, similar to AlpaServe~\cite{li2023alpaserve}, we disable batching in this work.


\noindent \subsection{APIs.} \noindent\tianrui{Moved from Section: Implementation} We have implemented five APIs for the interaction with {\system} shown in Table \ref{tab:API}. \\
\textbf{Model registration.} Model developers register the model using the \texttt{register} API. It accepts model information in a format of \texttt{modelFamily, modelSize} and supported compression techniques \texttt{quantization(s)}, which model developers should ensure they won’t severely harm the quality of output. Then, {\system} starts generating the {\submodel}s and profiles the model. Once profiling is finished, the model is added to the supported model list so that users can see it using texttt{list} and deploy it.\\
\textbf{User inference.} Users get the available model using the \texttt{list} API that prints all already registered models. Then, users deploy a model using \texttt{deploy} by providing an ID that is associated with the model, a maximum output length, and a policy that will be used to select the most befitting configuration. After the model loads, Users send queries by using \texttt{inference} with the model’s associated ID. The model client processes each query and replies back to users. Once users finish their work with a given model, they can remove it and free the memory using \texttt{remove} by providing the associated ID.\\


\begin{table}[t]
\centering % to center the table
\small
\begin{tabular}{c|c} % Add vertical lines between columns
\hline % Top horizontal line
\textbf{API}                             & \textbf{Parameters}                                                               \\
\hline % Horizontal line between rows
list                &  -                                                                                                     \\
\hline
register            & \begin{tabular}{@{}c@{}}modelFamily, modelSize(s), quantization(s)\end{tabular}                        \\
\hline
deploy              & ID, model, maxOutputLength, policy                                                                     \\
\hline
inference           & ID, input                                                                                              \\
\hline
remove              & ID                                                                                                     \\
\hline % Bottom horizontal line
\end{tabular}
\caption{{\system}'s APIs.}
\label{tab:API}
\end{table}
% \prasoon{T\&D, include a few sentences here on why we dont' consider beyond batch size 1. Make sure to cite papers as required to justify why this is okay to do in our context.}
% \dimitrios{{\system} uses for all serving requests a batch size of 1, so each user can provide their queries one by one throughout the inference cycle. This mimics the behaviour of an online LLM serving system, where users provide sequentially their queries and receive the generated text in the same order, before proceeding to the next query. Furthermore, by increases the batch size, the total serving latency increases, while the memory footprint of the model surges dramatically (e.g., Llama-7b requires $2.31\times$ more GPU memory when increasing the batch size from 1 to 128), due to its KV-cache size.}
% \neeraja{Prasoon, take a look at D's fix.} \tianrui{Additional to this, AlpaServe explains its reason that it doesn't use large batch: Batching in our system increases GPU utilization and throughput, but its benefits are limited due to saturation from small batch sizes in large models, leading us to disable it for clearer results except in specific experiments. (See AlpaServe Section 4.5 https://arxiv.org/pdf/2302.11665) We may use a similar reason.}
% \dimitrios{

% \noindent Based on our takeaways from \S~\ref{sec:background}, we guide our design of {\system}, a distributed inference serving system for LLMs that can serve concurrently multiple models in a dynamic GPU-environment and determine the optimal configuration for deployment based on the \emph{users'} objectives: minimize latency, memory, cost, or GPU-time. {\system} is able to achieve this by using three main components:
% \begin{enumerate}
%     \item \textbf{{\Submodel} Generator:} The {\Submodel} Generator is used for creating a lightweight variant of a given model. \S~\ref{sec:model-architecture} explains the architecture of a decoder-based LLM, which consists of a customized \emph{embedding layer}, multiple repeating \emph{hidden layers}, a \emph{linear layer} with \emph{normalization} and an \emph{activation function}. Among these components, the \emph{hidden layers} contain the majority of the model’s parameters (e.g. in Llama-2-70B more than 95\% of its weights are concentrated in its \emph{hidden layers}). We take advantage of this fact to construct a {\submodel} of the model that has the same architecture but is significantly more lightweight. Detailed information of {\system}'s {\Submodel} Generator is presented in \S~\ref{sec:generator}

%     \item \textbf{Profiler:} Model parallelism and quantization techniques (\S~\ref{sec:config-params}) can significantly impact a model's performance and alter its memory footprint. When deploying a LLM for inference, both latency and memory have an important role. Therefore, the role of the Profiler is to create the Model Database, which contain latency and memory related information about a model's deployment. The Profiler utilizes the {\submodel} of the model to collect the required information with minimum overheads and construct the Model Database. Detailed information of {\system}'s Profiler is presented in \S~\ref{sec:profiler}
    
%     \item \textbf{Model Deployer:} In \S~\ref{sec:config-params} we demonstrated how TP, PP, \& quantization have a different effect on total memory consumption, per-GPU memory consumption, and per-request latency. In a dynamic GPU environment both total and per-GPU memory have a significant role (e.g. a cluster might consist of a few large GPU or multiple small GPUs), especially when serving multiple models concurrently, where fragmentation is more likely to appear. On that account, we implemented the Model Deployer that receives the user-selected model alongside with their objectives, if any, creates a list of all possible configurations accompanied by their latency and memory information, derived from the Model Database, sorts them based on the objective and deploys the model with the most befitting feasible configuration based on the current memory availability of the GPU cluster starting from the least utilized GPU. Detailed information of {\system}'s Model Deployer is presented in \S~\ref{sec:deployer}.
% \end{enumerate}

% Figure ~\ref{fig:system_design} describes {\system}'s design and workflow. {\system} consists of four components: (a) the {\Submodel} Generator, (b) the Profiler, (c) the Model Deployer, and (d) the Scheduling Agent. These components are organized into two phases: (a) the Model Registration Phase, where a model is registered and profiled, and (b) the User Inference Phase, where users select a model and specify their objectives for inference serving. The workflow of {\system} is as follows: \textbf{1.} The \emph{developers} provide the pre-trained models that have to be profiled alongside with model-specific information (i.e., model's family, model's size, and applicable quatization techniques). \textbf{2.} The {\Submodel} Generator creates the {\submodel}'s fingerprint. \textbf{3.} The Profiler uses the model's {fingerprint} to collect latency and memory related information for every possible configuration and stores them into the Model Database. \textbf{4.} Then, \emph{users} can selected models from the pre-profiled list and specify their objectives. \textbf{5.} The Model Deployer will use the Model Database and Backend Cluster to determine the most optimal configuration, based on the objective, for the selected model and deploy it. \textbf{6.} Once the model is deployed, \emph{users} can invoke the deployed model by submitting requests. \textbf{7.} Finally, the Scheduling Agent receives the request from all online-users, populates the serving queue, and returns the result to them once they have been served.  

% The Model Registration Phase is intended to be decoupled from the User Inference Phase, so as not to be present on the critical path. Therefore \emph{users} do not have to incur
% the overhead of profiling a selected model. This requires that the Model Database is up-to-date when a \empph{user} selects a model for inference. In order to ensure that, the two phases can run concurrently on the same server, as our profiling algorithm ensures very small profiling costs, both in terms of latency and memory usage (\S~\ref{sec:eval_overhead}).
% }



==> 4_generator_profiler.tex <==
\section{{\Submodel} Generator \& Profiler}
\label{sec:generator_profiler}
\tianrui{From \S~\ref{sec:design}, we understand the importance of profiling among configurations for serving LLMs aligned with user objectives. However, directly loading LLMs and profiling across configurations is extremely expensive, consuming up to hundreds of gigabytes of memory. Therefore, leveraging the model architecture of LLMs as described in \S~\ref{sec:background}, {\system} generates and profiles the fingerprint—the essence of the entire model—using the Fingerprint Generator and Profiler, allowing for an estimation of the entire model at a lower cost.}
{\system} employs its Fingerprint Generator and Profiler when a user registers an LLM with {\system}.
The Fingerprint Generator creates two lightweight variants of the user's LLM while maintaining its overall architecture.
The Profiler then uses the LLM's fingerprints to obtain metadata that it can use to trivially calculate the expected inference latency and GPU memory requirements of an LLM under a given deployment configuration.
We heavily optimize the Profiler to obtain this metadata within minutes with minimal GPU memory requirements.
This enables {\system}'s Profiler to leverage the marginal spare memory left in the \emph{online} GPU cluster for profiling; {\system}'s Profiler does not require dedicated GPUs.
We first describe how {\system} generates fingerprints for each LLM, followed by the methodology of our Profiler to obtain the metadata required to calculate latency and memory requirements trivially at deployment time.

\subsection{{\system}'s Fingerprint Generator}
\label{sec:fingerprints}

\prasoon{TODO: we need to specify that we extract the number of parameters}

{\system}'s Fingerprint Generator constructs the \emph{fingerprint} of an LLM, a lightweight variant of the model that encapsulates its unique architecture in a much smaller memory footprint.
\S~\ref{sec:background} details the standard model architecture used across unique decoder-only LLMs.
The key components that bloat the memory footprint of LLMs and that LLMs spend the most time in during inference are the identical hidden layers, which do\prasoon{blah} \dimitrios{perform complex transformations and computations for processing the input tokens and generating the output human-like text.}.
We find a linear relationship between the number of hidden layers and memory footprint/inference latency; that is, increasing an LLM's hidden layer count increases its memory footprint and inference latency by a predictable, fixed amount (Figure ~\ref{fig:fingerprint_scaling}).
\prasoon{Do we have any data to show this in a graph or table of some sorts?}. \dimitrios{Done}
We take advantage of this repetitive, predictable nature of the LLM architecture to build a small fingerprint of the LLM, enabling {\system} to gather all its necessary profiling data for the LLM within minutes with little GPU memory consumption.

The Fingerprint Generator takes the original LLM as an input and creates two fingerprints of the LLM.
It first breaks down the LLM's unique components: an embedding layer, stacked hidden layers, a linear layer with normalization, and an activation function (Figure ~\ref{fig:fingerprint}).
It then constructs two fingerprints, $F_1$ and $F_2$, with all the unique components of an LLM, but with a minimal number of hidden layers:\emph{only one and two hidden layers}, respectively.
Hence, the fingerprint is more lightweight and fast, requiring a fraction of the memory and time for inference serving (e.g., Llama-2-70B's \prasoon{give stat on how much smaller and faster here in terms of $x\times$ with respect to memory and inference speed} \tianrui{fingerprints consume $30.85\times$ less memory and $33.68\times$ less time when serving a single request.})
Importantly, by maintaining the unique components of the original LLM architecture, {\system} can apply the same compression techniques and tensor parallelism as the original model, which {\system}'s Profiler takes advantage of.
We note that because we remove most hidden layers, PP degrees $>2$ (using $F_2$ with two hidden layers) cannot be applied, as there is simply not enough layers to distribute over more than two GPUs. \dimitrios{Should we mention here that this does not affect any of our results?}
\prasoon{Once you write in section 3 at the end why we only consider batch size 1, then we can see what to include here.}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/4.Profiler/fingerprint_scaling.pdf}
    \caption{Both latency and memory scale linearly as the number of hidden layers in the {\submodel} increases, as tested with Llama-2-7b generating 100 tokens. \tianrui{Update.}}
    \label{fig:fingerprint_scaling}
\end{figure}










\subsection{Estimating Inference Latency per Deployment Configuration}
\label{sec:latency-profiling}
\tianrui{Given an LLM and a configuration, {\system} needs to determine the latency of serving a request with arbitrary output lengths. Intuitively, this is challenging to profile because the latency varies by output length, as LLMs use an autoregressive decoding mechanism that generates output token by token. When serving a request, \Circled{1} the model first computes all input tokens and produces the first token. Then, for each output token, \Circled{2} the newly generated token is fed back into the model to calculate the output token. However, the use of a KV cache enables us to calculate the latency for any output lengths without exhaustive profiling, because the KV cache avoids recomputing preceding tokens, ensuring that the generation time for each token in \Circled{2} after the first one remains consistent.}
\noindent\textbf{Using a system of linear equations.} The latency of a single LLM request is dictated by three variables: the time to produce the first token ($TTFT$), the time to produce each output token ($TPOT$), and the output length (i.e., the number of tokens the LLM must generate):
\begin{equation}
\label{eq:lat}
latency = TTFT + output\_length \times TPOT
\end{equation}
Each inference request can have different output lengths, however $TTFT$ and $TPOT$ are \emph{specific to an LLM's deployment configuration}.
For a given LLM configuration $c$, its $TTFT_c$ and $TPOT_c$ can be decomposed into the latencies to go through the LLM's building blocks (e.g., hidden layers, other layers \S~\ref{sec:background}):
\[TTFT_{c} = num\_layers \times TTFT_{layer} + TTFT_{other}\]
\[TPOT_{c} = num\_layers \times TPOT_{layer} + TPOT_{other}\]
where \(num\_layers\) is the number of hidden layers in the LLM, \(TTFT_{layer}\) is the latency through one hidden layer to produce the first token, \(TPOT_{layer}\) is the latency through one hidden layer to produce an output token, and \(TTFT_{other}\) and \(TPOT_{other}\) are the latencies of the other basic building blocks for their respective token generation.
With knowledge of these values per configuration, {\system} can trivially calculate the latency for any inference with a specified output length under a given LLM deployment configuration using the aforementioned equations. 
\tianrui{All these parameters are included in the essence of the model, which can be obtained by utilizing fingerprints instead of the entire model.}
Thus, our Profiler's objective is: for all deployment configurations $c$ for a given LLM, efficiently obtain $TTFT_{layer}$, $TPOT_{layer}$, $TTFT_{other}$, and $TPOT_{other}$.

To reduce the memory consumed during profiling to obtain these values, we use the LLM's two fingerprints $F_1$ and $F_2$ which contain one or two hidden layers, respectively, along with the other unique LLM components (e.g., embedding layer, linear layer).
For each fingerprint under a given deployment configuration, we observe the E2E latency to serve an inference with two different output lengths.
Then, using equation (1), we decompose the latency of each output length of each fingerprint to create a linear system of four equations with four unknowns. Subscripts denote the fingerprint (F1) followed by the output length observed (O1)
\[latency_{F1O1} = TTFT_{F1} + output\_length_{F1O1} \times TPOT_{F1}\]
\[latency_{F1O2} = TTFT_{F1} + output\_length_{F1O2} \times TPOT_{F1}\]
\[latency_{F2O1} = TTFT_{F2} + output\_length_{F2O1} \times TPOT_{F2}\]
\[latency_{F2O2} = TTFT_{F2} + output\_length_{F2O2} \times TPOT_{F2}\]
As we specify all four output lengths and observe all four latencies, we trivially calculate $TTFT_{F1}$, $TTFT_{F2}$, $TPOT_{F1}$, and $TPOT_{F2}$.
Finally, since fingerprints $F1$ and $F2$ have one and two hidden layers respectively, we use the calculated values from the system of equations to calculate $TTFT_{layer}$, $TPOT_{layer}$, $TTFT_{other}$, and $TPOT_{other}$ for a given configuration.
\[TTFT_{layer} = TTFT_{F2} - TTFT_{F1}\]
\[TPOT_{layer} = TPOT_{F2} - TPOT_{F1}\]
\[TTFT_{other} = TTFT_{F1} - TTFT_{layer}\]
\[TPOT_{other} = TPOT_{F1} - TPOT_{layer}\]

\noindent\textbf{Optimizing latency profiling time.}
{\system}'s Profiler repeats the process of observing fingerprint latencies and solving a system of linear equations for each configuration the LLM can be deployed under.
Observing four inference latencies using an LLM's fingerprints (as opposed to the entire LLM) reduces GPU memory requirements for profiling.
We further optimize our profiling by reducing the number of configurations we need to observe.
\prasoon{T\&D, write two-three sentences here explaining how you do this. Make sure to explain you use PP = 1, why you don't have observe the LLM's fingerprints under different PP configurations (cite papers for this), and what are the configuration parameters that you change for each configuration that you observe. Also specify a worst case on the number of configurations you observe across the models. } \tianrui{In inference serving with a batch size of 1, communication between pipeline stages is minimal. Additionally, the latency caused by unbalanced layer assignments is absent since no micro-batch is used. The overhead from pipeline parallelism in serving the Llama-2-70B model constitutes less than 0.1\% of the total time. Consequently, we do not profile every pipeline parallelism level; instead, we use data from PP=1 for any level of pipeline parallelism or layer assignment, disregarding the negligible overheads. This approach significantly reduces the maximum number of profiles needed for one model to 32. }
\prasoon{This explanation lacks a few things. 1) We haven't specified anywhere the fact that we are only considering batch size 1. Why do we do that in this work? 2) What is a microbatch? We haven't mentioned it up to this point in the paper. 3) You mention some numbers (0.1\%). Where does that come from? Can you cite papers to back this up? Is this from your experiments? If so, is there data you have?} \dimitrios{(1) We do that because we consider the serving system as a one-shot executor, let's say that we have multiple users accessing ChatGPT, each of those will ask a question and get their answer back, in the order they were submitted. Moreover, we disregard the batches as they do not serve any purpose to our implementation because we don't take advantage of the batch size in the Scheduler (if we had a more sophisticated Scheduler, then it could collect all the single batch queries and create a larger batch to be served, increasing the overall throughput, but increasing total latency too). You are right, the first time we mention that the batch size 1 is in the evaluation, but we don't exactly know where is a good place to mention it. (2) Gpipe \cite{huang2019gpipe} was the first paper to propose the micro-batches. Basically when PP is applied each batch must go sequentially from one gpu to the next, by breaking the batch into micro-batches, they were able to reduce PP latency as each gpu could start processing the next micro-batch as soon the first had finished, without having to wait for the whole batch to be processed. In our case, however, we only have a batch size of 1 so using a micro-batch cannot reduce the bath further. (3) The number is from our measurement study.}


\subsection{Profiling Memory per Deployment Configuration}
\label{sec:memory-profiling}
\tianrui{When utilizing different parallelism and compression techniques, {\system} needs to know the memory requirements of each configuration to ensure they fit within environmental constraints. Parallelism techniques increase memory consumption because unsplittable parts need to be replicated. In profiling, {\system} specifically profiles these parallelism overheads in addition to the memory required by the model.}
The memory footprint of LLMs grows with larger parallelism degrees (\S~\ref{sec:background}), as components of the LLM are replicated across the GPUs depending on the type of parallelism(s) employed.
Figure ~\ref{fig:memory_overheads} illustrates the total memory consumption of an LLM under different parallelism configurations~\cite{luo2023rtp}.
The memory footprint of a model with no parallelism is simply the combination of its weights and activations.
TP replicates the activations of each layer on each GPU, inflating the memory footprint from the base LLM by $(N_{TP}-1) \times A$, where $N_{TP}$ is the TP degree and $A$ is the memory footprint of the activations.
PP replicates the intermediate PP activations on each GPU, increasing the LLMs footprint by $N_{PP}\times A_{P}$, where $N_{PP}$ is the PP degree and $A_P$ is the footprint of the PP activations.
Finally, a combination of TP and PP incurs overheads of both TP and PP.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/4.Profiler/parallel_overhead.pdf}
    \caption{Memory overhead of different Parallelization Strategies on LLMs. $N_{TP}$ and $N_{PP}$ refer to tensor and pipeline parallelism degree respectively, $A$ and $W$ refer to the activation and weight memory, $A_P$ is the intermediate activation of a pipeline layer.}
    \label{fig:memory_overheads}
\end{figure}
% \vspace{-2.5pt}

Across the four types of parallelism configurations, there are three constant values: the memory footprint of the weights $W$, the memory footprint of the activation $A$, and the memory footprint of the intermediate PP activation $A_P$. 
These values are fixed across different parallelism degrees $N$.
Hence, with knowledge of these values, {\system} can trivially calculate the memory requirements of any deployment configuration for an LLM.
Thus our Profiler's objective is: for a given LLM, efficiently obtain the memory footprint of the LLM's weights, activations, and intermediate PP activations.

Similar to latency profiling, \tianrui{we notice that the parallelism overhead profiled from fingerprints can be used to estimate the entire model.}we reduce the time and memory consumed during profiling by only observing the memory consumption of the LLM's two-layer fingerprint $F_2$ under three unique deployment configurations: no parallelism (i.e., TP = 1, PP = 1, LLM placed on a single GPU), TP = 1 and PP = 2, and TP = 2 and PP = 2.
We pick these parallelism configurations to observe multiple combinations of TP and PP degrees while keeping the required GPUs to profile low.
% \prasoon{T\&D, give a one sentence explanation on why these three configurations (out of many configuration options) were chosen -- reasons should include that it requires the least GPUs as well.} \dimitrios{Those configurations were selected as we wanted to observe the memory footprint under multiple combinations of TP and PP while keeping the number of utilized GPUs as low as possible.}
% \prasoon{Why not TP = 2, pp = 1? that requires fewer GPUs than TP = 2 and PP = 2. Explain that as well.}
% \dimitrios{Althought we could have picked TP = 2 \& PP = 1 as the third unique configuration, we deemed more appropriate the choice of TP = 2 \& PP = 2 as it can capture the concurrent effect of TP and PP.}
With the know memory consumption and parallelism degrees for each configuration, {\system} solves a linear system of equations (three equations from Figure ~\ref{fig:memory_overheads}), to obtain the values of $W$, $A$, and $A_P$ for each LLM.


==> 7_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

\noindent We conduct a series of experiments using real-world traces to evaluate {\system} and answer the following questions:

% \begin{enumerate}[label=\Roman*.]
%   \item How much does {\system} improve latency performance and resource utilization compared to baselines?
%   \item How well does {\system} achieves the \emph{user’s} objectives?
%   \item How well {\system} performs under limited GPU resources in serving LLMs?
%   \item How much is {\system}'s performance affected when reducing the configuration space?
%   \item How accurate is {\system} in estimating latency and memory usage?
%   \item What is the impact of on-fleet profiling?
%   \item What is the impact of the \emph{buffer\_size} on inference serving?
% \end{enumerate}
\noindent\textbf{Q1: }\textit{How much does {\system} improve latency performance and resource utilization compared to baselines?} (Section~\ref{sec:eval_end_to_end})\\ 
\noindent\textbf{Q2: }\textit{How well does {\system} achieve the \emph{user’s} objectives?} (Section~\ref{sec:eval_end_to_end})\\
\noindent\textbf{Q3: }\textit{How much is {\system}'s performance affected when reducing the configuration space?} (Section~\ref{sec:eval_limited_config})\\
\noindent\textbf{Q4: }\textit{How well does {\system} perform under limited GPU resources in serving LLMs?} (Section~\ref{sec:eval_limited_env})\\
\noindent\textbf{Q5: }\textit{How accurate is {\system} in estimating latency and memory usage?} (Section~\ref{sec:eval_estimation})\\
\noindent\textbf{Q6: }\textit{What is the impact of on-fleet profiling?} (Section~\ref{sec:eval_overhead})\\
\noindent\textbf{Q7: }\textit{What is the impact of the \texttt{buffer\_size} on inference serving?} (Section~\ref{sec:eval_sensitivity})\\
%\subsection{Methodology}
%\label{sec:eval_methodology}
\noindent \textbf{Testbed.} We deployed {\system} on a cluster with \textit{8× NVIDIA RTX A6000 (48GB each) GPUs}. Each pair of GPUs is connected with NVLINK, while the remaining connections utilize PCIe. The cluster features an AMD EPYC 7763 64-Core Processor, Ubuntu 22.04, and NVIDIA Driver 535.171.04 with CUDA Version 12.2. The TensorRT-LLM, on which {\system} relies, is built and executed in a Python session without using NVIDIA Docker.

% Are we still using the synthetic trace??
\noindent \textbf{Models and Workload.} We evaluate {\system} using both real and synthetic traces. For the real-world trace, we selected Azure's LLM inference trace 2023~\cite{patel2024splitwise}, a production trace for LLMs that consists of two different one-hour traces: (a) the \emph{conversation} trace with a steady and high load, and (b) the \emph{code} trace with a fluctuating load. Both of those contain information about the timestamp of an invocation with the respective input and output sizes. To scale the trace, we calculate the number of requests per minute, adjust the number by a scaling factor, and generate the corresponding number of requests for each minute block using a uniform distribution every 30 seconds. The synthetic trace that we utilized consists of invocations, following a uniform distribution, which were generated using a constant number of RPM throughout the experiment. To simulate a real-world production scenario, we deployed state-of-the-art models (Table ~\ref{tab:eval_models}) of varying sizes from three model families. We assume all models are stored in the TensorRT-LLM format. Each incoming request randomly selects a deployed model, mimicking the behavior of users accessing models randomly. The requests utilize the ShareGPT dataset ~\cite{sharegpt}, which records a collection of user-shared conversations with ChatGPT ~\cite{openai2024chatgpt}. Throughout this evaluation, the batch size is set to one, unless indicated differently.

\begin{table}[t]
\centering % to center the table
\small
\begin{tabular}{|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}} \textbf{Model}\\\textbf{Family} \end{tabular} &
\begin{tabular}[c]{@{}c@{}} \textbf{Model}\\\textbf{Size} \end{tabular} &
\begin{tabular}[c]{@{}c@{}} \textbf{Parallelism}\\\textbf{Technique} \end{tabular} &
\begin{tabular}[c]{@{}c@{}} \textbf{Quantization}\\\textbf{Technique} \end{tabular} \\
\hline
Llama-2 ~\cite{touvron2023llama}      & 
\begin{tabular}[c]{@{}c@{}} 7B, 13B,\\ 70B \end{tabular} & PP, TP  & \begin{tabular}[c]{@{}c@{}} INT8, INT4, GPTQ4, \\INT8 KV Cache \end{tabular}  \\
\hline
Falcon ~\cite{almazrouei2023falcon}   & 7B, 40B      & PP, TP      & INT8, INT4                        \\
\hline
GPT-J ~\cite{gptj}                    & 6B           & PP, TP      & INT8, INT4   \\                     
\hline
\end{tabular}
\caption{Models and supported configurations used throughout the evaluation.}
\label{tab:eval_models}
\end{table}

\noindent \textbf{Evaluation Metrics.} As a serving system, the SLO attainment of latency is a crucial metric for assessing service quality. We evaluate the latency SLO attainment of {\system} along with various baselines across different workloads and SLOs to demonstrate {\system}'s capability to support multiple LLMs. The default latency SLO of each model is set to $5\times$ of its single request latency with the simplest configuration (i.e., minumum TP, PP and no quantization), which is a tight SLO. Also the default rate scale for the LLM traces is set to $0.1x$ which corresponds to a rather bursty workload. {\system} is designed to meet user-defined objectives, which may include minimizing cost, latency, memory usage, or GPU hours. Hence, we also evaluate several performance metrics of {\system} under various constraints and objectives. These metrics include (a) total GPU memory usage, (b) resource utilization measured by the number of utilized GPUs, and (c) the number of models that can be loaded onto the cluster before triggering an Out-Of-Memory (OOM) error.


\noindent\textbf{{\system}'s policies}. In the evaluation, we assess our four implemented policies. First, the minimizing memory setting, \emph{min\_mem}, aims to reduce the memory usage for each model. Second, the minimizing latency setting, \emph{min\_lat}, focuses on reducing the inference latency of a single request. Third, the minimizing cost setting, \emph{min\_cost}, aims to reduce both inference latency and memory usage, simulating the user's goal of optimizing resource usage and task completion time. Finally, the minimizing gpu time setting, \emph{min\_gpu\_hour}, aims to reduce the amount of GPUs for the time it takes to serve an inference query.

% We might omit HF baselines
\noindent \textbf{Baselines.} We compare {\system} with two static baselines, one state-of-the-art inference systems, and one state-of-the-art inference framework (Table ~\ref{tab:eval_baselines}), as summarized below:

\begin{enumerate}
  \item \textit{PP-baseline}: It applies the maximum PP configuration to all models using the TensorRT-LLM framework, simulating the default setting in the transformer’s library ~\cite{huggingface}.
  \item \textit{TP-baseline}: It involves applying the maximum TP configuration to all models using the TensorRT-LLM framework.
  \item \textit{Alpa} ~\cite{li2023alpaserve}: It implements the \emph{Alpa} ~\cite{zheng2022alpa} algorithm that solves an NLP problem of parallelism configuration using communicating cost to determine the deployment of models. This is an alternative version implemented on the TensorRT-LLM framework.
  \item \textit{HF-\{Bal, Seq\}}: \emph{HuggingFace} (HF) ~\cite{huggingface} provides the users with an automated deployment method for LLMs using the Fully Sharded Data Parallel (FSDP) ~\cite{zhao2023pytorch} technique that shards a model's states across multiple GPUs. The two most prominent mapping configuration are: (a) the \emph{Balanced} configuration which distributes equally the states across all the available GPUs and (b) the \emph{Sequential} configuration which starts by occupying sequentially the available GPUs. Both of those are available through the \emph{Accelerate} ~\cite{sylvain2022accelerate} library.
\end{enumerate}

\begin{table}[t]
\resizebox{\linewidth}{!}{%
\centering
% \small
\begin{tabular}{l|cccc}
\toprule
\textbf{Features} & 
\begin{tabular}[c]{@{}l@{}} \textbf{TensorRT-LLM} \end{tabular} & 
\begin{tabular}[c]{@{}c@{}} \textbf{TensorRT-LLM} \\ \textbf{+ Alpa} \end{tabular} & 
\textbf{HuggingFace} & 
\textbf{{\system}} \\ 
\hline
Auto Parallelization  & \textcolor{red!70!black}{No} & \textcolor{yellow!50!black}{Static} & \textcolor{yellow!50!black}{Static}  & \textcolor{green!50!black}{Dynamic} \\
Auto Compression      & \textcolor{red!70!black}{No} & \textcolor{red!70!black}{No}        & \textcolor{red!70!black}{No}         & \textcolor{green!50!black}{Yes}     \\
Auto Device Selection & \textcolor{red!70!black}{No} & \textcolor{red!70!black}{No}        & \textcolor{green!50!black}{Yes}      & \textcolor{green!50!black}{Yes}     \\
User-defined Policy   & \textcolor{red!70!black}{No} & \textcolor{red!70!black}{No}        & \textcolor{red!70!black}{No}         & \textcolor{green!50!black}{Yes}     \\
\bottomrule
\end{tabular}
} %
\caption{Comparison between {\system} and the baselines.}
\label{tab:eval_baselines}
\end{table}


% Answer to Q1 and Q2
\subsection{{\system} with production workload}
\label{sec:eval_end_to_end}

We start with an end-to-end comparison of {\system} against all the baselines. For this experiment, we have used Azure's LLM inference trace with multiple scale factors and we deploy four models with the following sequence: Llama-2-70B, Falcon-40B, Llama-2-7B, and another Falcon-40B. These models are served using incoming requests driven by Azure's LLM inference trace, where each incoming request randomly picks a loaded model. The input length is capped at 1024 tokens, and the output length is limited to 20 tokens. Each model is deployed sequentially every five minutes during the trace replay. When a new model is loaded, we pause incoming requests for 60 seconds to facilitate the loading process. For comparing the collected results we have used three metrics: (a) The SLO attainment, (b) the total GPU memory usage, and (c) the maximum number of GPUs that were used on the model deployment process. Overall, \emph{{\system} consistently achieves the highest SLO attainment while reducing the total GPU memory and the number of wasted resources.}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/7.Evaluation/E2E_NO_SLO_full.pdf}
    \caption{Placeholder...}
    \label{fig:end-to-end}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/7.Evaluation/eva_7_1.pdf}
    \caption{SLO-attainment under various settings. In the first row, we scale the trace to simulate different arrival rates. In the second row, we modify the SLO scale that represents different SLO standards. \textit{pp\_baseline} and \textit{HF\_seq} are not shown because they received an OOM error.}
    \label{fig:end-to-end}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/7.Evaluation/eva_7_1_mem.pdf}
    \caption{The memory consumption and maximum GPU usage of models in the end-to-end evaluation.}
    \label{fig:mem_and_gpu}
\end{figure}

\noindent \textbf{\{TP, PP\} - Baselines.} The TP and PP baselines mimic the behavior of a non-expert user, that would have used the maximum TP and PP degree, respectively. Figure ~\ref{fig:end-to-end} shows that \emph{tp\_baseline} perform similarly to our policies for extremely low rate scales and loose SLO standards. As the invocations become more fluctuating and the SLOs are tightened we notice a decrease in the SLO attainment. Figure ~\ref{fig:mem_and_gpu} shows that \emph{tp\_baseline} requires $3.99\times$ more GPU memory compared to our \emph{min\_mem} and \emph{min\_gpu\_hour} policies, due to the float precision. While our system is able to exploit quantization for reducing the memory usage, \emph{tp\_baseline} can load the model only in \emph{float16} precision. For \emph{pp\_baseline} and \emph{HF\_seq}, the data is omitted because the inference cycles could not be completed due to an OOM error when deploying the models.

\noindent \textbf{Alpa.} The \emph{alpa} baseline performs similarly to the \emph{tp\_baseline}. As stated before, as the invocations become more fluctuating and the SLOs are tightened we notice a decrease in the SLO attainment. In Figure ~\ref{fig:mem_and_gpu} we can see that the \emph{alpa} baseline requires the most amount of memory to deploy all the selected model (i.e., $4.17\times$ compared to our best policies). Once again, this is caused by the limitation of the \emph{alpa} policy to take advantage of the float precision type and quantize the model. Furthermore, \emph{alpa} uses a max number of 8 GPUs to deploy a single model, which account to $8\times$ the amount that \emph{min\_mem} and \emph{min\_gpu\_hour} require, leading to significant waste of resources.

\noindent \textbf{HuggingFace Baselines.} The \emph{HF\_bal} and \emph{HF\_seq} baselines, overall, perform the worst. On the one hand, \emph{HF\_bal} cannot finish a request within the selected limits even for significantly low rate scales and for very loose SLOs, while increasing the wasted resources, as it needs all of the available GPUs for each model deployment. Its only advantage is that it requires less total GPU memory compared to \emph{alpa} and \emph{tp\_baseline}. On the other hand, \emph{HF\_seq} receives an OOM error, when deploying the bigger LLMs due to poor GPU management; it tries to allocate GPU memory agnostic to the cluster-availability so when specific parts of layers cannot be divided, an OOM error arises.

{\system} outperforms all the baselines on the SLO attainment, total GPU memory usage, and utilized GPUs. Our policies can successfully minimize latency, memory usage, GPU time, and overall cost by deploying the models in the most optimal configuration based on the user's objective. Regarding the SLO-attainment (see Figure ~\ref{fig:end-to-end}), the \emph{min\_lat} and \emph{min\_cost} policies perform relatively the same while outperforming all of the other policies and baselines. The SLO attainment stays for the majority of the time above the 80\% threshold and only drops below that for extremely fluctuating invocations. In Figure ~\ref{fig:mem_and_gpu} we can see that {\system}'s policies utilize only a fraction of the available GPU memory while reducing the number of wasted GPUs. The \emph{min\_mem} policy uses $4.17\times$ less GPU memory compared to \emph{alpa}, while the \emph{min\_gpu\_hour} policy uses a maximum of 1 GPU on model deployment, which is 7 fewer GPUs compared to the 8 GPUs used by \emph{alpa} and \emph{tp\_baseline}.


% \subsection{{\system}'s Response to User's Objectives}
% \label{sec:eval_objectives}


\subsection{{\system} with fixed compression technique}
\label{sec:eval_limited_config}

We show that {\system} can reach good SLO attainment and ensure the quality of service by utilizing only the parallelism techniques. In this section, we evaluate {\system}’s performance when the quantization is fixed by the user, which leaves {\system} with only the option of utilizing the parallelism techniques to achieve a user’s goal. For this experiment, we deployed all models using only a pre-selected precision: (a) only \emph{float16} (Figures ~\ref{fig:end-to-end-float16-INT4} \& ~\ref{fig:mem_and_gpu-float16-INT4}) and (b) only \emph{INT4} (Figure ~\ref{fig:end-to-end-float16-INT4} \& ~\ref{fig:mem_and_gpu-float16-INT4}). In the \emph{float16} experiment, we use the same settings as in Section \ref{sec:eval_end_to_end}. In the \emph{INT4} experiment, the baselines with \emph{INT4} weights use less space, allowing us to load more models and deliver a comprehensive evaluation of multi-model serving. Consequently, we added three more models: GPT-J-6B, Falcon-7B, and Llama-2-13B to the trace and we increased the output length across the models by 50 tokens. We have also omitted the \emph{alpa} baseline because it cannot use quantization. Overall, \emph{{\system} can still achieve different objectives based on policies in optimizing latency, memory, or cost while maintaining good quality of service.}

\noindent \textbf{Float16.} When using only \emph{float16}, {\system} faces a slight degradation in the SLO-attainment, which can be explained by the fact that the increased model sizes incur an extra overhead in the inference latency. Our \emph{min\_lat} policy has an SLO attainment close to that of the \emph{alpa} and \emph{tp\_baseline} baselines but requires less total GPU memory, $5.84\%$ and $0.86\%$ respectively. However, our \emph{min\_mem} and \emph{min\_gpu\_hour} policies can save up to $1.16\times$ and $1.11\times$ GPU memory compared to  \emph{alpa} and \emph{tp\_baseline} and only use $2.89\%$ more compared to \emph{HF\_bal}, while requiring a maximum number of only 4 GPUs for each model deployment compared to the whole cluster that all other baselines need.

\noindent \textbf{INT4.} For the \emph{INT4} experiment, the increase in the numbers of models used, increases the overall workload and that subsequently causes a delay on serving the requests. Due to that, we can notice that the SLO attainment degrades significantly across all policies and baselines. However, {\system} outperforms all other baselines across all the metrics. The \emph{min\_lat} and \emph{min\_cost} policies achieve the highest SLO attainment, while the \emph{min\_mem} and \emph{min\_gpu\_hour} policies can save up to $1.5\times$ of GPU memory compared to the static baselines. \emph{HF\_bal} and \emph{HF\_seq} have a near zero SLO attainment, however they show a slight advantage on reducing the total GPU memory, $1.95\%$ and $3.18\%$ respectively, compared to out \emph{min\_mem} and \emph{min\_gpu\_hour} policies, but in the expense of more wasted resources.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/7.Evaluation/eva_7_2_all.pdf}
    \caption{SLO-attainment under various settings when the quantization of all models is limited to INT4 or Float16.
    }
    \label{fig:end-to-end-float16-INT4}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/7.Evaluation/eva_7_2_all_mem.pdf}
    \caption{The memory consumption and maximum GPU usage when the quantization of all models is limited to INT4 or Float16.}
    \label{fig:mem_and_gpu-float16-INT4}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/7.Evaluation/eva_7_2_INT4.pdf}
%     \caption{SLO-attainment under various settings when the quantization of all models is limited to INT4.
%     }
%     \label{fig:end-to-end-INT4}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/7.Evaluation/eva_7_2_INT4_mem.pdf}
%     \caption{The memory consumption and maximum GPU usage of models when using only INT4.}
%     \label{fig:mem_and_gpu_float16}
% \end{figure}


\subsection{{\system} in limited resources}
\label{sec:eval_limited_env}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/7.Evaluation/eva_7_3_model_loads.pdf}
    \caption{Number of models loaded before receiving an OOM error for different policies.}
    \label{fig:eval_limited_env}
\end{figure}

We now show that {\system} has the ability to fully utilize the GPU resources and load a massive number of LLMs to serve. For each {\system} policy or baseline, we sequentially deploy models from Table~\ref{tab:eval_models} in a cycle until we receive an OOM error. This simulates that users deploy multiple LLMs on a resource-constraint server. In order to fairly compare {\system} against the baselines with more models, we have manually set the float precision of the baselines to \emph{INT4} to ensure minimal memory consumption of each model. Figure ~\ref{fig:eval_limited_env} shows the number of models deployed to a 4-, 6-, and 8-A6000 GPU cluster. Overall, {\system} can deploy $1.4\times$ more LLMs compared to the baselines using the \textit{min\_mem} and \textit{min\_gpu\_hour} policies which optimize the memory usage. \textit{min\_lat} and \textit{min\_cost} also show an advantage in deploying more models but their advantages are limited because optimizing latency by applying parallelism requires more memory. {\system} outperforms the baselines because (a) {\system} can dynamically pick the number of GPUs for each model based on the policy, and (b) {\system} can pick a sub-optimal configuration to fit the model in the server when the available memory is limited. 


\subsection{Profiler's latency and memory estimation error}
\label{sec:eval_estimation}

As described in \S~\ref{sec:deployer}, when {\system} tries to find the most optimal deployment configuration, the first step is to make an estimation of the serving latency and the memory footprint of all possible ones, based on the metadata collected from the Profiler. We show, here, that {\system} can make those predictions with very small errors.  

Figure \ref{fig:mem_lat_prof} presents the distribution of the errors, for the three model families, when predicting inference latency and memory footprint for various configurations. Regarding the latency prediction, the average prediction error for all the models is $5.4\%$, which corresponds to less than $50$ms of inference time. The latency prediction is feasible for predicting the overall inference latency for any output length while reducing both the time and memory required for profiling. Our method can save an average of $16.10\times$ of max GPU memory consumption and $3.56\times$ of profiling time compared to profiling the large-size LLMs. Regarding the memory prediction, the results indicate that our estimations have an average error of $12.58\%$ across all models %were able to achieve MAPE scores from 2.18\% to 12.56\%
; more significantly, for the larger LLMs, Falcon-40b and Llama-70b, the predictions errors are $5.60\%$ and $2.63\%$, respectively. The actual value of memory misprediction across all models is between 1.84 GB and 2.88 GB. By using the {\submodel} memory profiling we were able to reduce the cost both latency-wise and memory-wise. The average reduction in memory usage is $11.73\times$ and the average reduction in profiling latency is $3.86\times$.

\begin{figure}[t]
     \centering
        \includegraphics[width=\linewidth]{Figures/7.Evaluation/latency_n_memory_est_error.pdf}
        \caption{Memory and latency prediction error for each model family across different parallelism and compression techniques. }
        \label{fig:mem_lat_prof}
\end{figure}



\subsection{On-fleet Profiling}
\label{sec:eval_overhead}

{\system} enables on-fleet profiling to register and profile a new model using the same cluster that is concurrently serving LLM inference requests. The Profiler's usage of {\submodel}s significantly reduces the memory and time required to complete the profiling while having minimal impact on the current LLMs' serving performance. Figure ~\ref{fig:profiling_combined} shows a case study where {\system} starts profiling the Llama-2-70B model while serving the Llama-2-13B model. The arrival pattern follows Azure's LLM inference trace \textit{conversation} with a rate scale of 0.05, and the maximum output token count is 50. Figure ~\ref{fig:profiling1} shows the end-to-end time of each request in serving, with some requests being delayed by a few seconds because the Profiler preemptively occupies the cluster for model loading and inference. More than 50\% of the requests are not impacted by the on-fleet profiling. This demonstrates that the on-fleet profiling does not significantly affect the Quality of Service (QoS) of {\system}. Figure ~\ref{fig:profiling2} shows the maximum allocated GPU memory during the on-fleet profiling. Here, profiling Llama-2-70B using {\submodel}s saves $5.22\times$ more memory compared to profiling the entire Llama-2-70B model.

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/7.Evaluation/on_fleet_profiling_1.pdf}
        \caption{The end-to-end latencies of single serving requests.}
        \label{fig:profiling1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/7.Evaluation/on_fleet_profiling_2.pdf}
        \caption{The memory consumption of various settings.}
        \label{fig:profiling2}
    \end{subfigure}
    \caption{The impact of on-fleet fingerprint profiling in {\system} when profiling the Llama-2-70B model while serving the Llama-2-13B model.}
    \label{fig:profiling_combined}
\end{figure}


\subsection{Sensitivity study}
\label{sec:eval_sensitivity}

\begin{table}[t]
\centering
\small
\begin{tabular}{|c|c|c|}
\hline
\textit{buffer\_size} & single request latency (s) & Free memory left (GB) \\
\hline
1\% & 1.49 & 43.81 \\
\hline
10\% & 1.69 & 45.95 \\
\hline
\end{tabular}
\caption{The performance of the last Falcon-40B model deployed with different \textit{buffer\_size}.}
\label{tab:sensitivity}
\end{table}


{\system} uses a hyperparameter \texttt{buffer\_size} that reserves a portion of the GPU memory that is withheld when making deployment decisions. This buffer is used to account for potential memory under-prediction from using the memory profiling metadata and to leave some free space for the dynamic memory required for the KV-cache when serving a query. The default \texttt{buffer\_size} in {\system} is set to 10\% of the available GPU memory. This decision was data-driven, as the average memory mispredictions were about 10\%. The results in Table~\ref{tab:sensitivity} show the decisions made by two \texttt{buffer\_size} hyperparameters when deploying the last Falcon-40B model with the \textit{min\_lat} policy, using the same models as described in Section~\ref{sec:eval_end_to_end}. A \texttt{buffer\_size} of 1\% allows the model to be deployed using the optimal configuration for minimizing latency. A \texttt{buffer\_size} of 10\% chooses a configuration that reduces the level of parallelism to save unused memory space in each GPU. A smaller \texttt{buffer\_size} is preferred to allow more models to be deployed in the optimal configurations.


==> miscellaneous.tex <==
% Algorithm for {\Submodel} Generator
\begin{algorithm}[t]
\caption{{\Submodel} Generator: $fing\_gen(X, Y)$}
\label{alg:generator}
\begin{algorithmic}[0]
\small
\INPUT The whole-model's path $m\_path$, The {\submodel}'s number of hidden layers $n\_layers$
\OUTPUT The {\submodel}'s architecture ${\submodel}$
\STATE ${\submodel}$ $\gets \{\emptyset\}$
\STATE $model$ $\gets$ \textbf{LOAD} whole-model from $m\_path$
\STATE $building\_block\_list$ $\gets$ \textbf{GET} building blocks of $model$
\FOR{$building\_block$ \textbf{in} $building\_block\_list$}
    \IF{$building\_block$ \textbf{is} hidden\_layer}
        \STATE ${\submodel}$ $\gets$ \textbf{APPEND} $building\_block \times n\_layers$
    \ELSE
        \STATE ${\submodel}$ $\gets$ \textbf{APPEND} $building\_block$
    \ENDIF
\ENDFOR
\RETURN ${\submodel}$
\end{algorithmic}
\end{algorithm}


% Algorithm for Latency Profiler
\begin{algorithm}[t]
\caption{Latency Profiler: $lat\_prof(X, Y, Z)$}
\label{alg:lat_prof}
\begin{algorithmic}[0]
\footnotesize
\INPUT The model's path $m\_path$, Supported TP configuration $TP\_list$, Supported quantization configuration $Q\_list$,
\OUTPUT The model latency database $model\_db\_lat$
\STATE $model\_db\_lat$ $\gets \{\emptyset\}$
\STATE $num\_of\_GPUs$ $\gets$ \textbf{GET} number of GPUs in the cluster
\STATE $num\_layers$ $\gets$ \textbf{GET} number of hidden layers from $m\_path$
\STATE \textit{// Generate 1-layers \& 2-layers {\submodel}}
\STATE ${\submodel}\_1$ $\gets$ $fing\_gen(m\_path, 1)$
\STATE ${\submodel}\_2$ $\gets$ $fing\_gen(m\_path, 2)$
\STATE \textit{// Profile each configuration using fingerprints}
\FOR{$(tp,q)$ \textbf{in} $TP\_list \times Q\_list$}
    \STATE $CONFIG$ $\gets$ [\text{TP}=$tp$, \text{PP}=1, \text{Q}=$q$]
    \STATE $CG\_1$ $\gets$ \textbf{BUILD} graph using ${\submodel}\_1$ with $CONFIG$
    \STATE $t\_1\_i$ $\gets$ \textbf{SERVE} a queries using $CG\_1$ with output\_length i
    \STATE $t\_1\_j$ $\gets$ \textbf{SERVE} a queries using $CG\_1$ with output\_length j
    \STATE $CG\_2$ $\gets$ \textbf{BUILD} graph using ${\submodel}\_2$ with $CONFIG$
    \STATE $t\_2\_i$ $\gets$ \textbf{SERVE} a queries using $CG\_2$ with output\_length i
    \STATE $t\_2\_j$ $\gets$ \textbf{SERVE} a queries using $CG\_2$ with output\_length j
    \STATE \textit{// Construct and solve the system-of-equation (s-o-e)}
    \STATE $TPOT$, $TTPT$ $\gets$ \textbf{SOLVE} s-o-e using the latency data
    \STATE \textit{// Append the data for all possible pipeline parallelism level}
        \FOR{$i$ \textbf{from} 1 \textbf{to} ($num\_of\_GPUs$ / $tp$)}
            \IF{$i$ \textbf{>} $num\_layers$}
                \STATE ${cnf\_i}$ $\gets$ [\text{TP}=$tp$, \text{PP}=$i$, \text{Q}=$q$]
                \STATE $model\_db\_lat$ $\gets$ \textbf{APPEND} $(m\_path, cnf\_i, TPOT, TTPT)$
        
            \ENDIF
        \ENDFOR
\ENDFOR
\RETURN $model\_db\_lat$
\end{algorithmic}
\end{algorithm}


% Algorithm for Memory Profiler
\begin{algorithm}[t]
\caption{Memory Profiler: $mem\_prof(X)$}
\label{alg:mem_prof}
\begin{algorithmic}[0]
\footnotesize
\INPUT The whole-model's path $m\_path$
\OUTPUT The model memory database $model\_db\_mem$
\STATE $model\_db\_mem$ $\gets \{\emptyset\}$
\STATE \textit{// Generate 2-layers {\submodel}}
\STATE ${\submodel}$ $\gets$ $fing\_gen(m\_path, 2)$
\STATE \textit{// Load and Profile 3 configurations}
\STATE $mem\_data$ $\gets \{\emptyset\}$
\FOR{$CONFIG$ \textbf{in} \{ [\text{TP}=1, \text{PP}=1, \text{PP\text{-}MAP}=(1)], \\ \hspace{60} [\text{TP}=1, \text{PP}=2, \text{PP\text{-}MAP}=(1,1)], \\ \hspace{60} [\text{TP}=2, \text{PP}=2, \text{PP\text{-}MAP}=(1,1)] \}}
    \STATE $CG$ $\gets$ \textbf{BUILD} graph using {\submodel} with $CONFIG$
    \STATE $M$ $\gets$ \texbf{SERVE} a query using $CG$ and collect memory info
    \STATE $mem\_data$ $\gets$ \textbf{APPEND} $M$
\ENDFOR
\STATE \textit{// Construct and solve the 3x3 system-of-equation (s-o-e)}
\STATE $mem\_base\_fing$, $tp\_cst$, $pp\_cst$ $\gets$ \textbf{SOLVE} s-o-e using $mem\_data$
\STATE $mem\_base$ $\gets$ \textbf{CALCULATE} weights-only memory for whole-model
\STATE $model\_db\_mem$ $\gets$ \textbf{APPEND} $(m\_path, mem\_base, tp\_cst, pp\_cst)$
\RETURN $model\_db\_mem$
\end{algorithmic}
\end{algorithm}


% Algorithm for Model Deployer
\begin{algorithm}[t]
\caption{Model Deployer: $model\_deploy(X, Y, Z, W, U)$}
\label{alg:deployer}
\begin{algorithmic}[0]
\footnotesize
\INPUT The model for deployment $model$, The output lenght $out\_l$, The optinional user defined policy $policy$, {\system}'s model database $mod\_db$, The working GPU environment $cluster$
\OUTPUT The deployed model $deployed\_model$
\STATE $deployed\_model$ $\gets \{\emptyset\}$
\IF{$policy$ \textbf{is} $None$}
    $policy$ $\gets$ $min\_cost$
\ENDIF
\STATE $num\_of\_GPUs$ $\gets$ \textbf{GET} number of GPUs in the $cluster$
\STATE $num\_layers$ $\gets$ \textbf{GET} number of hidden layers of $model$
\STATE $TP\_list$ $\gets$ \textbf{FIND} all possible TP configs for $model$ in the $cluster$
\STATE $PP\_list$ $\gets$ \textbf{FIND} all possible PP configs for $model$ in the $cluster$
\STATE $Q\_list$ $\gets$ \textbf{FIND} all possible Quant configs for $model$ 
\STATE $KV\_Q\_list$ $\gets$ \textbf{FIND} all possible KV-cache Quant configs for $model$
\STATE \textit{// Find all possible configurations}
\STATE $pos\_config\_info$ $\gets \{\emptyset\}$
\FOR{$(tp,pp,q,kv\_q)$ \textbf{in} $TP\_list \times PP\_list \times Q\_list \times KV\_Q\_list$}
    \STATE $config$ $\gets$ $(tp,pp,q,kv\_q)$
    \STATE $lat$ $\gets$ \textbf{CALCULATE} latency for $config$ with $out\_l$ from $mod\_db$
    \STATE $mem$ $\gets$ \textbf{CALCULATE} memory for $config$ from $mod\_db$
    \STATE $pp\_map$ $\gets$ \textbf{DISTRIBUTE} $num\_layers$ given the $cluster$ state
    \STATE $pos\_config\_info$ $\gets$ $[tp, pp, pp\_map, q, kv\_q, (lat, mem)]$
\ENDFOR
\STATE $sort\_pos\_config\_info$ $\gets$ \textbf{SORT} $pos\_config\_info$ based on $policy$
\STATE $best\_cofig$ ← $sort\_pos\_config\_info[0][:5]$
\STATE $deployed\_model$ $\gets$ \textbf{DEPLOY} $model$ using $best\_cofig$
\RETURN $deployed\_model$
\end{algorithmic}
\end{algorithm}
